Reviewing Labels: Label Graph Network with Top-k Prediction Set for Relation Extraction

The typical way for relation extraction is fine-tuning large pre-trained language models on task-specific datasets, then selecting the label with the highest probability of the output distribution as the final prediction. However, the usage of the Top-k prediction set for a given sample is commonly overlooked. In this paper, we first reveal that the Top-k prediction set of a given sample contains useful information for predicting the correct label. To effectively utilizes the Top-k prediction set, we propose Label Graph Network with Top-k Prediction Set, termed as KLG. Specifically, for a given sample, we build a label graph to review candidate labels in the Top-k prediction set and learn the connections between them. We also design a dynamic $k$-selection mechanism to learn more powerful and discriminative relation representation. Our experiments show that KLG achieves the best performances on three relation extraction datasets. Moreover, we observe that KLG is more effective in dealing with long-tailed classes.

==> 5-discussion.tex <==
\section{Other Explorations}\label{discussion}

\subsection{Using the \textit{Top-k} Prediction Set in Different Ways}
As a pioneering work of using the \textit{Top-k} prediction set, we also conduct some explorations. Under the assumption that we already have the \textit{Top-k} prediction set for each example, there are several simple and straightforward ways to utilize this information. We mainly consider the following two aspects: 
\begin{itemize}
    \item \textbf{Which paradigm should we use? Classification-based methods or generation-based methods?} Classification-based methods are the most popular paradigm for RE, but they simply treat the label as a one-hot vector and optimize parameters using cross-entropy loss. This procedure ignores the semantic information existing in the relation names, i.e., \textit{place of birth} and \textit{place of death} have a strong semantic correlation, but classification-based methods can not learn any useful information from the one-hot label vectors. Although some works \cite{} utilize hierarchical information of the classes, this information often needs human effort and is not always available for all datasets. On the contrary, generation-based methods directly treat relation names as generation objectives, and the model could learn some semantic information existing in relation names from the encoder-decoder architecture. With this ability, generation-based methods have the potential to use the \textit{Top-k} prediction set effectively.

    \item \textbf{Where should we inject the \textit{Top-k} prediction set to the model? At the Input or the Output?} The \textit{Top-k} prediction set is a set of alternative classes, and we can use it either at the input or the output. At the input, we can write a prompt and give some clues to the model. The prompt contains the \textit{Top-k} prediction set and some natural language, which may be helpful for the model to understand the available information existing in the \textit{Top-k} prediction set. Meanwhile, we can use the \textit{Top-k} prediction set at the output. For the classification-based methods, we use label smoothing to force the model to pay attention to the labels in the \textit{Top-k} prediction set. The idea of label smoothing was first proposed by Inception-v2 \cite{DBLP:conf/icml/IoffeS15}. It changes the one-hot label vector into a soft label. Intuitively, label smoothing restraints the logit value for the correct class to be closer to the logit values for other classes. As for the generation-based methods, instead of simply generating the relation name, we force the model to generate the \textit{Top-k} prediction set as well. By doing so, the encoder-decoder architecture may learn helpful information from the \textit{Top-k} prediction set.
\end{itemize}

\subsection{Model Design}
Based on the above discussion, we build the following four models: 

\textbf{1) Classification-based Method with Input Enhancement (CI).} In this setting, we use the base model introduced in \S \ref{comparison} as the encoder. Besides, we use prompt to inject the \textit{Top-k} prediction set into the input. Specifically, for a given example and its \textit{Top-k} prediction set \textit{s(Top-k)}, we add a prompt $P$ after the input text, and $P$ is: Choose a relation from \textit{s(Top-k)} for the $e_1$ and the $e_2$. Where $e_1$ and $e_2$ denote the head entity and tail entity.

\textbf{2) Classification-based Method with Output Enhancement (CO).} \textbf{CO} uses the \textit{Top-k} prediction set in the output. It uses the same backbone network as \textbf{CI}, and the input is the original input text without prompt. Besides, \textbf{CO} modifies the one-hot label as the soft label, and the loss $\mathcal{L}$ is computed as follows:
\begin{equation}
    \mathcal{L} = \gamma\mathcal{L}^{CE}(i) + \frac{1 - \gamma}{k}\sum_{j \in \textit{s(Top-k)}}\mathcal{L}^{CE}(j).
\end{equation}
Where $\gamma$ = 0.9 in our experiment. By using the soft label, \textbf{CO} could pay attention to the labels in the \textit{Top-k} prediction set.

\textbf{3) Generation-based Method with Input Enhancement (GI).} In this setting, we first use BART as the backbone network, and the input format is the same as \textbf{CI} with a minor modification: we randomly shuffle the orders of labels in \textit{s(Top-k)}. The purpose of this is to avoid BART from simply copying the first label in \textit{s(Top-k)} as the prediction. The generation objective of \textbf{GI} is the relation name. And the loss here is the sequential cross-entropy loss between the relation name and the model's output. \textbf{GI} may learn helpful information from the prompt and achieves better performance.


\textbf{4) Generation-based Method with Output Enhancement (GO).} We also design a model that uses BART and inject the \textit{Top-k} prediction set at the output. \textbf{(GO)} uses the original input text as input, and we force it to generate the ground truth first, then the model also needs to generate labels in the \textit{Top-k} prediction set one by one. With this setting, we hope the encoder-decoder architecture could learn the label correction from the generation objectives, and use the \textit{Top-k} prediction set effectively.

To help readers better understand our model design, we take a training sentence from TACRED as an example and show the detailed settings in the Appendix \ref{}. 

%The input sentence is: $x$ = \uline{ @ Lindsay Hayes @, a national \# specialist \# prison suicide prevention who ...}, the head entity and tail entity is \textit{Lindsay Hayes} and \textit{specialist}. The ground truth is \textit{per:title}, and the \textit{Top-6} prediction set \textit{s(Top-6)} is \textit{\{per:title, org:founded, org:shareholders, no\_relation, per:city\_of\_birth, per:age, per:spouse\}}. The inputs and outputs of different models are shown in Table \ref{}.

\begin{table}[h]
\centering
\setlength{\tabcolsep}{1.3mm}
\begin{tabular}{c|c|c|c}
\toprule[1.5pt]
\multicolumn{1}{c|}{Model} & Paradigm                        & Input/Output & Micro-F1            \\ \hline
RoBERTa-large              & \multirow{3}{*}{Classification} & -            & 74.3                \\ \cline{1-1} \cline{3-4} 
CI                         &                                 & Input        & 74.1(-0.2)          \\ \cline{1-1} \cline{3-4} 
CO                         &                                 & Output       & \textbf{74.6(+0.3)} \\ \hline
BART-large                 & \multirow{3}{*}{Generation}     & -            & 72.7                \\ \cline{1-1} \cline{3-4} 
GI                         &                                 & Input        & 72.0(-0.7)          \\ \cline{1-1} \cline{3-4} 
GO                         &                                 & Output       & \textbf{73.5(+0.8)} \\ \bottomrule[1.5pt]
\end{tabular}
\caption{The results using different model designs. We report the Micro-F1 score on the test set of TACRED. The number in the bracket is the performance change compared with the corresponding baseline model.}
\label{exploration}
\end{table}

\subsection{Experimental Results}

In this subsection, we report the experimental results on the test set of TACRED. Due to the space limitation, please refer to Appendix \ref{} for the experimental settings and training details. From Table \ref{exploration} we can observe that:
\begin{itemize}
    \item Directly injecting the \textit{Top-k} prediction set into the input could not achieve better performance as we expected, even with the help of prompt. \textbf{GI} even suffers 0.7\% Micro-F1 score degradation compared with its corresponding baseline model. We think there are two possible reasons for the above phenomenon: 1) the backbone network can not understand the meaning of semantic meaning of relation names, and appending the \textit{Top-k} prediction set after the input text may confuse the model's encoder, making the model pay less attention to the original input text. 2) With sufficient training samples, models may learn to select a relation name from the \textit{Top-k} prediction set directly without considering the original input text.
    
    \item We find that if we leverage the \textit{Top-k} prediction set at the output, the models could achieve considerable improvements, especially for the \textbf{GO}. As \textbf{GO} forces the decoder to generate both the ground truth relation name and the \textit{Top-k} prediction set, it may activate the power of BART's decoder and learn some semantic correlation between relation names, finally benefiting the performance.  
\end{itemize}

To sum up, \textbf{GO} has great potential to utilize the \textit{Top-k} prediction set and make considerable improvements. We leave this as future work. 

\subsection{The Difference with Partial Label Learning}

At the first glance, the usage of the \textit{Top-k} prediction set is similar to the Partial Label Learning (PLL) \cite{DBLP:journals/ida/HullermeierB06,DBLP:journals/jmlr/CourST11,DBLP:conf/kdd/ZhangZL16,DBLP:journals/corr/abs-2201-08984}. PPL assumes that each training example is equipped with a set of candidate labels instead of the exact ground truth label. In fact, they are totally different. One crucial difference is that PLL is a weakly supervised learning setting, since it doesn't have the ground truth for the training set. While our setting is a standard supervised learning paradigm. Besides, the PLL requires the ground truth label existing in its candidate label set, and the supervised single could only extract  from the candidate label set. While in our setting, we just treat the \textit{Top-k} prediction set as supplementary information, and do not need it must contains the ground truth label. Additionally, the candidate labels in PLL need human annotation, but the \textit{Top-k} prediction set in our experiment is automatically generated. 

It should be emphasized that it is possible to use the technique of PLL to improve the utilization of the \textit{Top-k} prediction set, and we leave this as future work. 

